UAV-based Maritime Communications: Relaying to Enhance the Link Quality

Providing a stable connectivity in maritime communications is of utmost importance to unleash the full potential of smart ports. Nonetheless, due to the crowded nature of harbor environments, it is likely that some ships are shadowed by others, resulting in reduced received power that subsequently diminishes their data rates-even threatens basic connectivity requirements. Given that uncrewed aerial vehicles (UAVs) have been regarded as an integral part of future generations of wireless communication networks, they can be employed in maritime communications as well. In this paper, we investigate the use of UAV-mounted relays in order to help mitigate the reduced data rates of blocked links in maritime communications. Various communication architectures are considered based on the positioning mechanism of the UAV; in this regard, fixed, k-means algorithm-based, and landing spot-based positioning approaches are examined. Additionally, since UAVs are predominantly battery-operated, the energy consumption performances of these approaches are also measured. Results reveal that the landing spot-based UAV relay positioning approach finds the best trade-off between the data rate and energy consumption.

==> cop_biography.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{taha_foto.jpg}}]
{\textbf{ABDULLAH TAHA ÇAĞAN}} was born in 2000 in Ankara.  He is currently studying at Ankara Yıldırım Beyazıt University, Ankara, Turkey, Faculty of Engineering and Natural Sciences, Department of Electrical and Electronics Engineering.  In 2022, he worked as a Visiting Researcher at Aalto University, Espoo, Finland.  His interests include energy management and indoor positioning in artificial intelligence networks and cellular communication systems.  
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{gorkem_photo1.jpg}}]
{\textbf{GÖRKEM BERKAY KOÇ}} is currently pursuing a B.Sc. degree in electrical and electronics engineering at Ankara Yıldırım Beyazıt University, Ankara, Turkey. He worked as a Visiting Researcher at Aalto University, Espoo, Finland in 2022. He was awarded as Study in Canada Scholarship (SICS) holder by Global Affairs Canada and he is currently working as a Visiting Researcher at Carleton University, Ottawa, Canada. His research interests focus on optimizing wireless communication network performance, non-terrestrial networks and high altitude platform station (HAPS) sustainability.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{handanyakin.jpg}}]
{\textbf{HANDAN YAKIN}} is currently pursuing a B.S. degree in electrical and electronics engineering with Ankara Yıldırım Beyazıt University, Ankara, Turkey. She worked as a Visiting Researcher at Aalto University, Espoo, Finland. Her research interests include wireless communications, signal space diversity, visible light communication, and Optical orthogonal frequency-division multiplexing (OFDM).  
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{foto_berk.jpg}}] 
{\textbf{BERK ÇİLOĞLU}} is currently pursuing a B.Sc. degree in electrical and electronics engineering at Ankara Yıldırım Beyazıt University, Ankara, Turkey. He worked as a Visiting Researcher at Aalto University, Espoo, Finland in 2022. As an awardee of the study in Canada scholarship (SICS) by Global Affairs Canada, he is currently working as a Visiting Researcher at Carleton University, Ottawa, Canada. 
His research interests lie in the area of wireless communication network performance optimization, non-terrestrial networks, and high-altitude platform station (HAPS) sustainability.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Zeeshan.png}}]
{\textbf{MUHAMMAD ZEESHAN ASGHAR}} is post-doctoral researcher
at the department of communication and networking, Aalto
University Finland. Muhammad completed his Ph.D. in
Wireless Communication at the University of Jyväskylä,
Finland in 2016. He has received a several awards, including
Future City Challenge (Jyväskylä) Winner 2018 and
conference paper award at ICEIC Barcelona 2019.
He was a principal investigator of BusinessFinland funded project of on 5G Cognitive Self-organizing Networks (CSON) at the University of Jyväskylä during the years 2017-2019. 
He raised 500K euro for the commercialization of his research on 5G. The project outcome is a startup company that provides R\&amp;D support to telecom vendor and mobile network operators on AI/ML powered network automation for 5G/6G networks.
Prior to this, Muhammad worked as a Research Engineer for Nokia-Siemens Networks Solutions, Finland during 2008-2014. During this work he wrote one patent that was granted in year 2016. His research interests in 5G/6G Radio Access Networks, OpenRAN Architectures, AI/ML based network automation, private 5G/6G networks and industrial IoT.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.3in,clip,keepaspectratio]{OE_foto.jpg}}]
{\textbf{ÖZGÜN ERSOY}} was born in Aydın, Turkey, in 1989. He received a B.S. degree in electronics and communication engineering from Kocaeli University, Kocaeli, Turkey in 2012, and an M.S. degree in electrical and electronics engineering from Ankara Yıldırım Beyazıt University, Ankara, Turkey in 2017. He is currently pursuing a Ph.D. degree with the Department of Electrical and Electronics Engineering, at Ankara Yıldırım Beyazıt University, Ankara, Turkey. His research interests include wireless communication, millimeter wave and terahertz frequency communication, modulation methods, and channel access methods.  
\end{IEEEbiography}

\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Jyri_Hamalainen.jpg}}]
{\textbf{JYRI HÄMÄLÄINEN}} is Full Professor of Aalto University, Finland. He received his M.Sc. and Ph.D. degrees from University of Oulu, in 1992 and 1998, respectively. From 1999 until the end of 2007 he was a Senior Specialist and Program Manager in Nokia where he worked with various aspects of mobile communication systems and 3GPP standardization. Hämäläinen was nominated to professor of Aalto University in 2008 and he was tenured in 2013. His research interests cover mobile and wireless systems, special focus being on irregular, dynamic and heterogeneous networks including e.g. 5G/6G, small cells, multi-antenna transmission and reception techniques, scheduling, relays and many other topics. Hämäläinen is author or co-author of 240 scientific publications and 37 US patents or patent applications. He is a Senior Member of IEEE. From 2015 Hämäläinen has been serving as a Dean in the Aalto University School of Electrical Engineering.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{metinozturk.jpg}}]{\textbf{METİN ÖZTÜRK}} received the B.Sc. degree in electrical and electronics engineering from Eskisehir Osmangazi University, Turkey, in 2013, the M.Sc. degree in electronics and communication engineering from Ankara Yildirim Beyazit University, Turkey, in 2016, and the Ph.D. degree from the Communications, Sensing, and Imaging Research Group, James Watt School of Engineering, University of Glasgow, U.K., in 2020. He worked as a Research Assistant (from 2013 to 2016) and a Lecturer (from 2020 to 2021) with Ankara Yildirim Beyazit University, where he is currently an Assistant Professor. His research interests include intelligent networking for wireless communication networks, with a focus on energy efficiency, mobility management, and radio resource management in cellular networks; he has authored \& co-authored 35+ research items, including journal papers, conference procedings, and book chapters.
\end{IEEEbiography}

